New results on the local linear convergence of ADMM: a joint approach

Thanks to its versatility, its simplicity, and its fast convergence, ADMM is among the most widely used approaches for solving a convex problem in distributed form. However, making it running efficiently is an art that requires a fine tuning of system parameters according to the specific application scenario, and which ultimately calls for a thorough understanding of the hidden mechanisms that control the convergence behaviour. In this framework we aim at providing new theoretical insights on the convergence process and specifically on some constituent matrices of ADMM whose eigenstructure provides a close link with the algorithm's convergence speed. One of the key technique that we develop allows to effectively locate the eigenvalues of a (symmetric) matrix product, thus being able to estimate the contraction properties of ADMM. In the comparison with the results available from the literature, we are able to strengthen the precision of our speed estimate thanks to the fact that we are solving a joint problem (i.e., we are identifying the spectral radius of the product of two matrices) in place of two separate problems (the product of two matrix norms).

==> CO16.tex <==
% !TEX root = ../co.tex

\definecolor{yellow}{RGB}{255,215,0}
\definecolor{yellow}{RGB}{200,200,200}
\definecolor{red}{RGB}{255,255,255}
\definecolor{orange}{RGB}{0,0,0}
\definecolor{yellow}{RGB}{0,0,0}
\definecolor{green}{RGB}{0,0,0}
\definecolor{red}{RGB}{0,0,0}
\definecolor{blue}{RGB}{0,0,0}
\definecolor{violet}{RGB}{0,0,0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unitlength = 1.8mm
\begin{center}\begin{small}

\begin{tikzpicture}[y=1mm,x=1mm,scale=3.5]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\draw[fill=black!10] (0,0) circle (4);
\draw(0,-4.5) [-latex] -- (0,6) node [anchor= west] {$\Im$};
\draw(-8,0) [-latex] -- (8,0) node [anchor= north] {$\Re$};

\draw[black,ultra thick] (0,0) circle (4);
\draw[black,ultra thick] (3.2,0) node (aa) {$\bullet$} node [below] {$\breve{p}$} -- (5,0) node (bb) {$\bullet$} node [below] {$\overline{p}$};
\draw[black,ultra thick] (-2.67,0) node (cc) {$\bullet$} node [below] {$-\breve{n}\;\,$}-- (-6,0) node (dd) {$\bullet$} node [below] {$-\overline{n}\;\,$};
\draw(1,4.5) node (gg) [right] {circle of radius $\overline{r}$};
\draw[dashed] (gg) [-latex] -- (3,3);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tikzpicture}


%%%%%
\end{small}\end{center}
\caption{Locus $\M N$ of the eigenvalues of $N(\alpha)$  in the complex plane (bold lines), under the assumptions of Theorem~\ref{teoremaAutovalFixed}.}
\endinput


==> CO26.tex <==
% !TEX root = ../co.tex

\definecolor{yellow}{RGB}{255,215,0}
\definecolor{yellow}{RGB}{200,200,200}
\definecolor{red}{RGB}{255,255,255}
\definecolor{orange}{RGB}{0,0,0}
\definecolor{yellow}{RGB}{0,0,0}
\definecolor{green}{RGB}{0,0,0}
\definecolor{red}{RGB}{0,0,0}
\definecolor{blue}{RGB}{0,0,0}
\definecolor{violet}{RGB}{0,0,0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unitlength = 1.8mm
\begin{center}\begin{small}

\begin{tikzpicture}[y=1mm,x=1mm,scale=20]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\draw[fill=black!10] (0,0) circle (4);
\draw(0,0) node [] {\includegraphics[width=60mm]{CO26b.pdf}};
\draw(1,-1.1) node [] {$n$};
\draw(-1.3,0.75) node [] {$\Gamma_n$};
\draw(0.5,0.1) node [rotate=-42] {$\rho_{\max}$ estimate};
\draw(0.3,-0.3) node [rotate=-32] {$\lambda^*_{\max}$ estimate};



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tikzpicture}


%%%%%
\end{small}\end{center}
\caption{Convergence measure $\Gamma = \|z^+-z\|$ versus the iteration number $n$, compared with the two speed estimates given by $\rho_{\max}$ (dashed lines) and $\lambda^*_{\max}$ (dash-dotted lines).}
\endinput

